Solvable models of two-level systems coupled to itinerant electrons: Robust non-Fermi liquid and quantum critical pairing

Strange metal behavior is traditionally associated with an underlying putative quantum critical point at zero temperature. However, in many correlated metals, e.g., high-Tc cuprate superconductors, strange metallicity persists at low temperatures over an extended range of microscopic parameters, suggesting the existence of an underlying quantum critical phase, whose possible physical origins remain poorly understood. Systematic investigations of physical scenarios giving rise to such a critical, non-Fermi liquid (NFL) phase are therefore crucial to better understand this puzzling behavior. In a previous work [Bashan et al. arXiv:2310.07768], we considered a solvable large-N model consisting of itinerant electrons coupled to local two-level systems (TLSs) via spatially random interactions, inspired by the possibility of emergent metallic glassiness due to frustrated competing orders, and found that the system hosts an NFL phase with tunable exponents at intermediate couplings. In this work, we expand our investigation to the following: (i) We study the extent to which this NFL phase is generic by considering various deformations of our theory, including coupling of electrons to multiple operators of the TLSs and arbitrarily directed TLS-fields. We find that the physical picture obtained in Bashan et al. qualitatively persist in a wide region of parameter space, showcasing the robustness of the NFL phase; (ii) We analyze the superconducting instability due to coupling of TLSs to electrons, and find a rich structure, including quantum critical pairing associated with the NFL phase and conventional BCS pairing in the weak and strong coupling limits; (iii) We elaborate on the analysis of Bashan et al., including single-particle, transport and thermodynamic properties.

==> old_summary.tex <==

\subsection{Old intro}


{\color{red} Understanding scenarios in which strong interactions between itinerant electrons and collective quantum fluctuations invalidate the conventional Landau Fermi liquid (FL) paradigm is a central problem in the field of correlated metals \cite{varma_colloquium_2020,chowdhury_sachdev-ye-kitaev_2021,hartnoll_planckian_2021,phillips_stranger_2022,sachdev_quantum_2023}. A prominent example of such a scenario is the enigmatic `strange metal' (SM) behavior found in high-$T_c$ superconductors and other quantum materials \cite{proust_remarkable_2019,bruin_similarity_2013,legros_universal_2019,cao_strange_2020}. SMs are commonly defined by an anomalous $T-$linear scaling of the dc resistivity at arbitrarily low temperatures, which directly contradicts the expected $T^2$ scaling predicted by FL theory.
%at very low temperatures. 
%Furthermore, w
While SM behavior is often associated with an underlying quantum critical point (QCP) at $T=0$ \cite{gegenwart_quantum_2008}, there are multiple examples, such as cuprates \cite{cooper_anomalous_2009,hussey_tale_2018,hussey_generic_2013,greene_strange_2020} 
, twisted bilayer graphene \cite{cao_strange_2020,jaoui_quantum_2022}, and twisted transition metal dichalcogenides \cite{ghiotto_quantum_2021}, where 
%SM behavior 
it appears to persist over an extended region, suggesting the interesting possibility of a critical, non-Fermi liquid phase 
%(or quantum critical phase) 
at zero temperature. %\noga{Maybe: Additional examples of observed extended NFL (but not SM) phases  are:} 
In addition, extended NFL behavior has been observed in MnSi with $T^{3/2}$ scaling of the resistivity \cite{pfleiderer_non-fermi_2003,pfleiderer_partial_2004,doiron-leyraud_fermi-liquid_2003,paschen_quantum_2021} and in CePdAl with a $T^n$ scaling with $n$ varying from $\sim1.4$ to $2$ \cite{zhao_quantum-critical_2019}.
%\joerg{didn't we have a dicussion on MnSi along with references? Seems to have disappeared... If we want to reintroduce this, we probably should also include this referebce https://www.nature.com/articles/s42254-020-00262-6} \evyatar{It's back with the new Paschen-Si reference}

The absence of a quasiparticle description in such systems, %In systems where FL theory is invalid, 
known as `non-Fermi liquids' (NFLs) \cite{anderson_new_1995,varma_singular_2002,lee_recent_2018} or `marginal Fermi liquids' (MFLs) \cite{varma_phenomenology_1989,varma_singular_2002},
%, is evidence of their intrinsic many-body nature which 
makes well-controlled theoretical investigations %considerably
challenging.
Nevertheless, recent years have witnessed a proliferation of illuminating solvable models, largely facilitated by the use of Large-$N$ and Sachdev-Ye-Kitaev (SYK) techniques \cite{sachdev_gapless_1993,Kitaev_SYK_talk,chowdhury_sachdev-ye-kitaev_2022,sachdev_quantum_2023}. In particular, the extensive analysis of a class of Yukawa-SYK theories \cite{marcus_new_2019, esterlis_cooper_2019,wang_quantum_2020,wang_solvable_2020,wang_phase_2021,esterlis_large_2021,guo_large_2022,valentinis_bcs_2023,valentinis_correlation_2023,patel_universal_2023}, where a Fermi surface is coupled to critical bosons, has demonstrated that strange metallicity can emanate from a quantum critical point (relying crucially on the presence of quenched disorder \cite{guo_large_2022,patel_universal_2023}). 

\begin{figure}[t]
\centering

 \includegraphics[width=1\columnwidth]{phaseDiagram_aTupdated.eps}

\caption{\textbf{Dynamical phase diagram of the $x-$model with a linear TLS distribution}. Dynamical phases in the $\alpha-T$ plane, where $T$ is measured in units of $h_c$ (the bare TLS cutoff energy scale) and $\alpha$ is the dimensionless coupling strength between the TLSs and the itinerant electrons. The colored area represents the low-$T$ dynamical regimes, characterized via the exponent $\gamma$ of the inelastic scattering rate (at $\Sigma''_R(\omega) - \Sigma_R''(0) \sim |\omega|^{\gamma}$). The $T$-dependent part of the resistivity is proportional to the inelastic scattering rate. The exponent $\gamma$ decreases with increasing the dimensionless coupling $\alpha$ ($\gamma = 2(1-\alpha)$), resulting  
%which is also bThe $T$-scaling of the resistivity obeys teh same formAt zero temperature, increasing the interaction strength, $\alpha$ changes the exponent in the resistivity temperature dependance, $\gamma=2(1-\alpha)$, resulting 
in FL behavior for $\alpha<1/2$, a MFL at $\alpha=1/2$ and a NFL for $\alpha>1/2$. As $\alpha$ crosses $1$, the TLSs  freeze one by one over a small range of $\alpha$'s. This collection of quantum phase transitions is indicated by a thick black line at $T=0$.  The low-$T$ regime persists up to temperatures of order $h_{R,c}(\alpha)$ (the renormalized TLS cutoff), represented by the dashed black line. This energy scale decreases as $\alpha$ increases, and goes to zero at $\alpha=1+h_c/\omega_c$. Above this temperature, the TLSs act as classical quasi-elastic scatterers with $T-$independent scattering rate (plus $T^2/E_F$ corrections), resulting in trivial FL behavior. The smooth crossover to this region is denoted by the fading out of the color.
}
\label{fig:phase diagram of x model}
\end{figure}

%shown that  in the presence of quenched disorder, strange metallicity can emanate from a quantum critical point.}has provided significant insights into the conditions under which strange metallicity can emanate from a quantum critical point, showing that quenched disorder plays a crucial role [xx].


%In contrast to theories of SM behavior that arise from fine-tuning, either QCP-induced strange metallicity, and despite manifest experimental evidence [new LSCO, tale of two metals, ...,xx] and some numerical evidence [Trembley QMC,...], 
In contrast to strange metallicity that arises due to tuning to a QCP,
%(or by neglecting relevant operators \cite{chowdhury_sachdev-ye-kitaev_2022}), 
a controlled microscopic theory hosting a stable NFL phase, free of fine-tuning,  remains noticeably absent within the existing literature. This is surprising as  such extended metallic critical phases seem to be allowed within  holographic setups \cite{zaanen_planckian_2019,hartnoll_horizons_2011}, and are also supported by numerical evidence \cite{wu_non-fermi_2022}.
%{\color{red}[MORE?]}.\joerg{I looked around but didn't really find other references}
Here, we show that a stable NFL phase can arise
%the possibility of strange metallicity arising 
due to coupling of electrons to the low-energy excitations of an underlying glassy order. This scenario draws inspiration from the intricate phase diagrams of high$-T_c$ superconductors which often exhibit a competition between multiple frustrated orders that could lead to metallic glassiness \cite{emery_frustrated_1993,kivelson_stripe_1998}. It is worth noting that such a scenario can arise independently of quenched disorder, namely, due to frustration-induced self-generated randomness \cite{schmalian_stripe_2000}. }
%which often contain  materials exhibiting SM behavior, where the competition of many frustrated orders could lead to glassy behavior.



%Here, we consider the possibility of strange metallicity arising due to coupling of electrons to the low-energy excitations of an underlying glassy order. This scenario draws inspiration from the intricate phase diagrams of high$-T_c$ superconductors which often exhibit a competition between multiple frustrated orders that could lead to metallic glassiness \cite{emery_frustrated_1993,kivelson_stripe_1998}. It is worth noting that such a scenario can arise independently of quenched disorder, namely, due to frustration-induced self-generated randomness \cite{schmalian_stripe_2000}. 
%which often contain  materials exhibiting SM behavior, where the competition of many frustrated orders could lead to glassy behavior. 

%Drawing inspiration from the intricate phase diagrams of high-$T_c$ superconductors, which often host multiple competing intertwined orders [xx], it seems natural to extend the search for NFL behavior to the following scenario. We imagine that the competition between frustrated orders leads to the formation of an electronic glass [maybe Emery+Kivelson ``frustrated...''], such that upon doping{\color{red} why mention doping here..?} we encounter a scenario where itinerant electrons are interacting with quantum glassy fluctuations. These fluctuations can be thought of as describing collective electronic excitations in a complex energy landscape that is characteristic of glassy systems [xx]. It is worth noting that such a scenario can arise independently of quenched disorder, namely, due to frustration-induced self-generated randomness [xx]. %Further, while we make no attempt to model any realistic material, the considered scenario is seems  there have 
%The main objective of this work is to investigate this intriguing scenario within a well-controlled non-perturbative theoretical framework.

To this end, the seminal works of Anderson, Varma and Halperin \cite{anderson_anomalous_1972} and Phillips \cite{phillips_tunneling_1972} showed that the low-energy collective excitations in a glass are effectively described by a collection of two-level systems (TLS). For a critical discussion of the TLS-phenomenology, see Ref.~\cite{leggett_tunneling_2013}. Each TLS represents a collective tunneling between nearby minima of the free energy associated with two nearly-degenerate configurations of a local collective mode. Quite generally, the level splitting and tunneling rate, characterizing each TLS, can be considered as independently distributed random variables due to their disordered nature. The  emergence of 
two-level systems (TLSs) in relation  to the unique energy landscape of glass-forming liquids was discussed in Refs.~\cite{lubchenko_intrinsic_2001,lubchenko_origin_2003}. 

\subsection{Results for the $x-$model}

We first consider a simple variant of the model, defined by $g_y^2=g_z^2=0$, $g_x^2 = g^2>0$ and $h_l^x \equiv 0$ 
%(or more precisely, $\mathcal{P}(h_x) = \delta(h_x)$ such that the TLS-splitting is parallel to the $z$ axis) 
for all $l$, dubbed the $x-$model. We set $V^2=0$ for simplicity, restoring it later on. Its sole effect is to provide an elastic scattering term. It turns out that  this variant can be mapped to the canonical Caldeira-Leggett SB model \cite{caldeira_quantum_1983,leggett_dynamics_1987,costi_thermodynamics_1999,weiss_quantum_2012}. It will provide useful intuition for more general variants we will consider later on. The dimensionless coupling strength, defined as $\alpha \equiv g^2 \nu^2_0 / \pi^2$ (to match the dimensionless coupling of the SB model, see Sec.~\ref{mappingtoTLSboson}), together with the exponent of the TLS-splitting distribution, $\beta$, constitute the main tuning parameters of the $x-$model. 

We find that that the \textit{local} particle-hole pairs that act as a bath to the TLSs are independent of the electronic self-energy. That is, while the TLSs renormalize the single-particle properties, the back-action of the electrons onto the TLS is independent of this renormalization, regardless of the coupling strength. This allows us to reduce the solution of our model to that of a single TLS;
%, similarly various `single-impurity' problems, e.g. [xx]; 
see Sec.~\ref{mappingtoTLSboson}.   


%where thermal fl
%at temperatures lower than the renormalized cutoff $h_{R,c}$, thermal broadening effects can be essentially ignored, such that the naive perturbative argument holds for the renormalized distribution, leading to a tunable exponent of the imaginary part of the electronic self-energy: $\Sigma_R''(\omega)\propto |\omega|^{(1+\beta)(1-\alpha)}$. 
%{\color{red} clarify that the above is derived from the Golden rule}

%Upon increasing the coupling to the vicinity $\alpha\approx 1$, the TLSs become frozen due to BKT transition, in which the effective scale becomes $ h_R\to0$, such that for $\alpha>1+h_c/\omega_c$ there are no more dynamical scatterers in the system, and the TLSs only contribute an inelastic scattering mechanism.

\begin{figure*}[t]
\centering

\includegraphics[width=2\columnwidth]{summaryofresultsREALLYNEW.eps}

\caption{\textbf{Summary of results for the $x-$model with bare linear splitting distribution $(\beta = 1)$}. (a) Dynamical regimes,
%of the model 
%at $T=0$ 
probed by the imaginary part of the retarded self energy (for $\alpha<1$). Upon increasing the coupling, $\alpha$, the electrons cross over from a Fermi liquid (FL) at weak coupling; to a marginal Fermi liquid (MFL) at $\alpha_{\rm MFL} = 1/2$; and onto a non-Fermi liquid (NFL) for $1/2<\alpha<1$. After a transition to a localized phase of the TLSs at $\alpha=1$, FL behavior is restored,
%the electrons revert back to Fermi liquid behavior 
albeit with additional static impurities (FL+SI). (b) The renormalized distribution of the effective splitting, $\mathcal{P}_r( h_R)$,  for increasing $\alpha$. (c) Imaginary part of the self energy for increasing values of $\alpha$, normalized by the saturation value $\Sigma_\infty \equiv \Sigma_R''(h_{R,c}\ll\omega\ll E_F)=\nu_Fg_x^2/2\pi $. The solid lines represent the power law behavior calculated in this work, and given in (a), while the dashed lines, starting around $\omega\simh_{R,c}$, schematically depict the approach to a saturation value. 
%{\color{red} maybe in (a) indicate more explicitly that this P~h is hte bare distribution?}
}
\label{fig:summaryofresults}
\end{figure*}


\begin{figure*}[t]
\centering

 \includegraphics[width=2\columnwidth]{Figs/ax_az_colormap.pdf}

\caption{\textbf{Schematic summary of results for the $xyz-$model with $\alpha_y=0$ and negligibly small $h_c/\omega_c$}. The exponent of the leading frequency dependent part of the self energy, $\gamma$, (defined by $\Sigma''_R(\omega \to 0) - \Sigma''_R(\omega = 0) \sim |\omega|^{\gamma}$) at zero temperature for a uniform (left) and linear (right) bare splitting distribution. Given any $\alpha_z$, by increasing $\alpha_x$ the electrons crosses over from a FL (blue), MFL (white), and NFL (red) behavior, until the TLSs undergo a BKT transition to a localized phase (denoted by solid black line) and turn into elastic scatterers restoring FL behavior. The dashed line denotes  $\alpha_x=\alpha_z$ where both couplings flow to weak coupling. Note that while the exact results we derive perturbatively in this work are valid only close to the axes, the schematic behavior at the non-perturbative regime is extrapolated based on the calculations performed by Ref.~\cite{kohler_nonequilibrium_2013}. 
%Replacing $\alpha_x\leftrightarrow \alpha_y$ does not change the picture and replacing $\alpha_z\leftrightarrow \alpha_y$ the top left half turns into a mirror image identical to the bottom right half (i.e. to $\alpha_z<\alpha_x$). 
%, and the solid black line indicates the BKT transition.
}
\label{fig:summary multibath}
\end{figure*}


\subsubsection{A simple view of the physical picture for $\alpha < 1$}

\label{simple view section}
Consider first the weak coupling limit, $\alpha \to 0$, where the effect of interactions can be studied perturbatively. To leading order in $g^2$ the decay rate of an electron with energy $\omega$ is proportional %electrons gain a self energy at zero temperature proportional 
to the amount of TLSs at accessible energies, namely, 
\begin{eqnarray}
\Sigma_R''\left(\omega\right)\propto \int_0^\omega \mathcal{P}_\beta \left(h \right) dh \propto |\omega|^{1+\beta},  
\end{eqnarray}
 $\Sigma_R''$ being the imaginary part of the electronic retarded self energy. For $\beta=0$ this weak coupling analysis yields marginal Fermi liquid behavior. On the other hand, for any $\beta>0$, i.e. for distribution functions that vanish  for $h\rightarrow 0$ one only finds Fermi liquid behavior.
 Increasing the strength of the interaction modifies the behavior of the TLSs in two main aspects: it renormalizes the energy splitting of each TLS, such that $h_\ell\to h_R(h_\ell)$; and broadens the TLS spectral function. The broadening has negligible effect on the frequency dependence of $\Sigma''_R$ (at sufficiently low energies). However, as we show in detail below,
 %the former  It turns out that at low enough temperatures the effect of the broadening is not important here, and the main effect is due to 
 the renormalization of the energy splitting leads to a renormalization of the bare TLS-splitting distribution: 
 %the interactions renormalize the bare TLS
%by a multiplicative factor  with a renormalized s factor that depends smoothly which leads to a renormalized splitting distribution $\mathcal{P}_{r,\beta}$. By virtue of the mapping to the Spin-Boson model, the renormalized distribution is a continuous function of the coupling strength, namely, $\mathcal{P}_{r,\beta}( h_R) = \mathcal{P}_{\beta-\alpha(1+\beta)}( h_R)$. 
\begin{eqnarray}
   \mathcal{P}_\beta(h) \to \mathcal{P}_{\beta-\alpha(1+\beta)}( h_R),
\end{eqnarray}
where $ h_R= h_R(h)$ denotes the renormalized splitting. That is, the exponent of the  distribution of splittings, $\beta$, decreases with increasing $\alpha$.
Increasing the interaction strength transfers the spectral weight of the TLSs toward lower energies (at the limit $\alpha \to 1$, the spectral weight is pushed to zero energy, signaling a BKT transition of the TLSs to a localized phase). See Fig.~\ref{fig:summaryofresults}(b) for an illustration of the evolution of $\mathcal{P}( h_R)$ for $\beta=1$. More details are given in Sec.~\ref{SBreview}.
%and in Fig.~\ref{fig:summaryofresults}(b), the evolution of $\mathcal{P}( h_R)$ is shown for $\beta=1$. 
%in the special case $\beta=1$: from a linear ($\alpha=0$), to a constant ($\alpha=1/2$), to $1/\log( h_R)$ ($\alpha=1$), and finally to a delta function centered at zero $(\alpha>1+h_c/\omega_c$) in the localized phase of the TLSs (see Sec.~\ref{SBreview})..
%Finally, 
%if the temperature is sufficiently low such that 
%is therefore expected that at sufficiently low temperatures, where 
%broadening effects can be ignored, 
Consequently, the naive perturbative argument will hold for the renormalized splitting distribution, resulting in a tunable exponent as a function of $\alpha$.
%: $\Sigma_R''(\omega)\propto |\omega|^{(1+\beta)(1-\alpha)}$.


\subsubsection{Dynamical regimes}

We characterize the dynamical regimes of the model with the imaginary part of the retarded self-energy. We begin with 
%We begin with the $T=0$ behavior at low energies, $\omega\ll h_{R,c}$, $h_{R,c}$ being the renormalized cutoff of the TLSs. 
$\alpha<1$, which corresponds to the dynamical (delocalized) phase of the TLSs, and find that at $T=0$:
\begin{equation} \Sigma_{R}''\left(\omega\right)=rA_\alpha \nu_{0}g^{2}\left|\frac{\omega}{h_{R,c}}\right|^\gamma,\quad \gamma \equiv (1+\beta)(1-\alpha).
\label{imagselfenergyalphaless1}
\end{equation}
Here the $\alpha$-dependent numerical coefficient $A_{\alpha} \sim \mathcal{O}(1)$ provided $\alpha < 1$ (see Sec.~\ref{alphalesonesubsc}), $\nu_0$ is the density of states at the Fermi level and $h_{R,c}$ is the renormalized cutoff of the TLSs, which is a decreasing function of $\alpha$ (so that the low-energy domain is reduced with increasing interaction strength). Interestingly, since the exponent $\gamma$ is a continuous function of the coupling strength $\alpha$, the self-energy can be tuned to realize a marginal Fermi-liquid form: $\Sigma_{R}''\left(\omega\right)\sim |\omega|$, provided that $\alpha = \alpha_{\rm MFL}\equiv \beta/(1+\beta)$ and $\beta>0$. The MFL behavior arises at generic couplings and is not associated with a quantum critical point \cite{sachdev_quantum_2011}, rather, the system smoothly crosses over between a Fermi liquid for $\alpha<\alpha_{\rm MFL}$ and a non-Fermi liquid for $\alpha>\alpha_{\rm MFL}$. 

%The case of linear splitting distribution is of special interest as it corresponds to a generic physical scenario, where $h_z$ is the eigenvalue of a $2\times2$ hamitlonian with two uniformly distributed parameters. 


Further increasing the coupling, $\alpha\geq1$, drives TLSs into a localized phase, where $\alpha=1$ is the critical BKT point of the SB model. At the critical point, $\Sigma_{R}''\left(\omega\right)\sim \log\left( \omega_c/|\omega|\right)^{-(1+\beta)}$, which intuitively follows from Eq.~\eqref{imagselfenergyalphaless1} as $\gamma\to 0$ for $\alpha \to 1$. Beyond the critical point, $\alpha>1$, there exists a small window, $1<\alpha<1+h_c/\omega_c$, where only the fraction of the TLSs with sufficiently small splittings ``freeze'' into a source of elastic scattering while the remaining TLSs obey a form similar to that at $\alpha=1$. For $\alpha>1+h_c/\omega_c$, all the TLSs are localized (i.e. static), such that the self energy is that of a Fermi liquid with static impurities (FL+SI). 



Recall that the case of a linear splitting distribution ($\beta=1$) is of special interest as it corresponds to the rotation to the diagonalizing basis where both $h^x,h^z$ are uniformly distributed. %scenario: Starting from an arbitrary basis, where it is reasonable to assume that $\boldsymbol{h}=( {h}_x,{h}_z)$ are generically distributed uniformly on a disk, the $\beta=1$ case corresponds the rotated axes where 
 Remarkably, for $\beta=1$, the MFL point ($\alpha=1/2$) coincides with the exactly solvable `Toulouse point' of the SB model \cite{anderson_exact_1970,leggett_dynamics_1987}, which enables us to obtain the exact MFL self-energy, see Sec.~\ref{TPfiniteT}. The dynamical regimes  of the $x-$model with $\beta=1$ are presented in Fig.~\hyperref[fig:summaryofresults]{\ref{fig:summaryofresults}(a,c)}. Note that at high-energies, the self-energy saturates to a constant value due to the bounded Hilbert space of the TLSs. The $T=0$ dynamical regimes described above extend to low temperatures ($T\ll h_{R,c}$), as we demonstrate explicitly at $\alpha=1/2$ (i.e. the `Toulouse point') for general $\beta$.
%and show that it holds for all $\alpha$ under reasonable physical assumptions on the TLS susceptibility; see Sec.~FINITE T.

Allowing for a field along $\hat{x}$ constitutes the simplest generalization of the $x-$model, dubbed the biased $x-$model (as it maps to the biased SB model). The bias, i.e. $h_x$, is unaffected by the interaction, while $h_z$ is renormalized as before. As a result, the self-energy admits an elastic contribution from the TLSs and the leading inelastic term takes the form $\Sigma_R''(\omega) - \Sigma_R''(0) \sim |\omega|^{ 1+\beta_x + (1 + \beta_z)(1-\alpha)}$. For the physically motivated case $\beta_x=\beta_z=0$ this corresponds to FL-like behavior for all values of $\alpha$, which approaches MFL-like behavior when $\alpha\to1$. 
%This is a simple example of the correspondence between the diagonalizing basis (with $\beta_z =1$ and $h_x \equiv 0$) and the physical basis (with $\beta_z =\beta_x = 0$).} 


\begin{comment}

{\color{red} add general finite temperature comment.} 

 
 Such behavior is presented in \ref{fig:summaryofresults}(c) for $\alpha=1+\epsilon$ where $\epsilon<h_c/\omega_c$. For $\alpha>1+h_c/\omega_c$, all TLSs are localized and contribute an elastic scattering term as depicted in Fig.~\ref{fig:summaryofresults}(c). Note also that at energies $\omega\gg h_{R,c}$, the scattering rate saturates to a constant due to the bounded Hilbert space of the TLSs. The approach to the saturation value is depicted schematically in dashed lines in Fig.~\ref{fig:summaryofresults}.





%, such that an increasing fraction of the TLSs constitute a source for elastic scattering, while the rest of the `delocalized' TLSs obey 



In FIGURE we display the corresponding "phase diagrams" for the most physical cases, $\beta=0,1$, along with the case in which we allow $\vec{h}=(h_x,h_z)$ to be distributed uniformly on a disk. The main effect of the interaction strength is thus to smoothly vary the exponent in the self energy, as well as to decrease the cutoff scale for the dynamical behavior, until complete freezing at $\alpha>1+h_c/\omega_c$.



    
\begin{itemize}
    \item Model does not admit a standard saddle-point analysis due to TLS. Instead, we employ a mapping to the Spin-Boson model, where we reduce the problem to that of $M$ decoupled TLS coupled to an Ohmic bosonic bath. {\color{red} refer to DMFT here?}
    
    \item The low-energy electronic properties of the model are determined by the dimensionless coupling strength, $\alpha = g^2\nu_0/\left(2\pi^2\right)$, and $\beta$, which sets the scaling of the TLS splitting distribution $\mathcal{P}(h) \propto h^\beta$.  
    \item Interaction renormalize the TLSs, leading to a renormalized distribution, which enters the electronic self-energy
    \item There is no backaction of the TLS onto themselves, namely, the TLS are acted on by a bath of non-interacting particle-hole pairs. 
    \item Scattering of the TLS is large-angle due to the spatially disordered couplings, such that transport times are proportional to the single-particle relaxation time. 
    \item The electrical resistivity $\rho = \rho_0 + AT^{2-2\alpha}$, and similarly for the thermal resistivity $\rho_{\rm th} = T/\kappa$ ($\kappa$ being the thermal conductivity. (In particular WF law is obeyed)...
\end{itemize}
\end{comment}


\subsection{Generalization to the $xyz-$model}

We move on to a more general case, where each TLS is allowed to interact with the electrons via arbitrary couplings $g_{a}^2>0$ for $a=x,y,z$ (for now keeping $h_x \equiv 0$, i.e. still working in the diagonalizing basis). By virtue of the mapping to the SB model, the dynamics of each TLS are now determined by a three-bath SB problem with ohmic baths and dimensionless couplings $\alpha_a$ for the $a-$bath. By analyzing the RG flow, we find that the low energy behavior of the $xyz-$model is effectively reduced to that of a single-bath. That is, it is generically the case that the bath with the largest bare coupling remains dominant at low energies, with a renormalized coupling $\alpha_a^r\lesssim\alpha_a$, while the other baths flow to weak coupling, resulting in subleading corrections to $\Sigma_R''$ (excluding potential elastic scattering terms, see Sec.~\ref{multibath-model section}).  

If the dominant bath is transverse to the field $h_z$ (i.e. $x-$ or $y-$baths), the dynamical regimes follow those of the $x-$model: assuming $a$ is the dominant bath, for $\alpha_a^r<1$ the leading inelastic part of the self energy is $\Sigma_R''(\omega)-\Sigma_R''(0) \sim |\omega|^\gamma$, with $\gamma=(1+\beta)(1-\alpha^r)$, while for $\alpha^r>1$ the TLSs freeze and become static impurities with finite-$T$ FL-like corrections. In this case, the coupling $\alpha_z>0$ induces an additional elastic scattering term, proportional to the equilibrium value $\langle \sigma_z \rangle ^2>0$ (see Sec.~\ref{multibath-model section}). However if the dominant bath is parallel to the field, at low energies the TLSs are nearly static with weak broadening due to the perturbative effects of the transverse baths. This leads to mostly elastic scattering of the electrons with subleading FL-like terms. 


Finally we consider a variant of the model where we allow a non-zero distribution of $h_x$ such that $\vec{h}$ points in an arbitrary direction in the $x-z$ plane. This variant, dubbed biased $xyz-$model, corresponds to setting the couplings to be uncorrelated in the physical basis (rather than the diagonalizing basis), and in that sense, might be the most natural variant of our model. As before, the behavior is determined by the direction of the dominant bath. If either $\alpha_x$ or $\alpha_z$ are the largest, the physical picture follows that of the biased $x-$model with the appropriate renormalized coupling. However if the $y-$bath dominates, the leading inelastic part of the self energy takes the form $\Sigma_R''(\omega)-\Sigma_R''(0) \sim |\omega|^\gamma$ with $\gamma=(2+\beta_x + \beta_z)(1-\alpha_{y,R})$ such that the physical picture follows that of the $x-$model. Remarkably, we see that an extended NFL phase persists in the most general variant of the model, provided that the $y$-bath dominates. \evyatar{restricted to alpha<1 comment}
%and in particular contains a NFL phase %without any fine tuning.
%\erez{In what sense is this ``less fine tuned'' than other cases?} \noga{Maybe fine tuned is not the correct term, but in the regular biased case the ׳׳MFL" only happens near $\alpha=1$ close to the transition to SIs.} \evyatar{Changed it a bit.} 
% In this case, we see the correspondence between the dynamical behavior in the diagonalizing basis (with $\beta_z = 1$ and $h_x \equiv 0$) and the physical basis (with $\beta_x = \beta_z = 0$).

\subsection{Transport and thermodynamics}

We focus on the dc resistivity and optical conductivity as the two main probes for transport, which we analyze using the Kubo formula. We find that the $T$-scaling of the dc resistivity, $\rho(T)$, follows that of the single-particle scattering rate. That is, considering for simplicity the $x-$model, for $\alpha<1$,
\begin{eqnarray}
    \rho(T\ll h_{R,c}) = \rho_0 + AT^{\gamma}, 
\end{eqnarray}
where the residual resistivity, $\rho_0$, is due to the on-site disorder term $V^2>0$, and $\gamma$ is given by Eq.~\eqref{imagselfenergyalphaless1}. In addition, the Wiedemann-Franz law is obeyed in the $T\rightarrow 0$ limit.
For $T\gtrsim h_{R,c}$, $\rho(T)$ saturates to a $T-$independent constant, similarly to $\Sigma_R''$ (up to a small $T^2/E_F$ correction). For $\alpha>1$, $\rho = \rho_0 + AT^2$, where now a portion of the residual resistivity is due to contribution of the frozen TLSs to the elastic scattering term. The $xyz-$model follows the same qualitative behavior provided that $z$ is not the dominant bath, and otherwise follow a FL-like behavior with enhanced residual resistivity as the dominant bath is that of approximately static TLSs. 

The optical conductivity contains a contribution from the itinerant electrons and a contribution from the dipole coupling of the TLSs to the electric field, such that $\sigma(\Omega) = \sigma_{\rm el}(\Omega) + \sigma_{\rm TLS}(\Omega)$. While the contribution from the itinerant electrons assumes a Drude-like form (see Sec.~\ref{opticalconductivity}), which is decreasing with $\Omega$, we find that the TLS contribution $\sigma_{\rm TLS}(\Omega)$ is an increasing function of $\Omega$ at low frequencies. This could give rise to non-monotonic frequency dependence of the optical conductivity $\sigma(\Omega)$, as shown in Fig.~\ref{fig:optical cond}. 
%{\color{purple} rephrase} either with one or two local minima for $\Omega\geq 0$ before approaching $0$ at high energies.


\begin{comment}such that
\begin{eqnarray}
        \sigma(\Omega) = \sigma_{\rm el}(\Omega) + \sigma_{\rm TLS}(\Omega). 
\end{eqnarray}
While the 
Restoring the on-site disorder $V^2>0$, for sufficiently small frequencies, $\sigma_{\rm el}(\Omega) \approx 1/\Gamma$, and the leading frequency dependence follow the optical conductivity 
\end{comment}
Evaluation of thermodynamic properties of the system is challenging due to the non-Gaussianity of the large-$N$ saddle point, which also precludes the use of Luttinger-Ward formalism. However, for the $x-$model, we use two alternative methods to verify that the temperature dependence of the specific heat assumes the form:
\begin{equation}
    C_v(T) \propto \begin{cases}
        T & \gamma>1, \\
        T\log{\frac{h_{R,c}}{T}} & \gamma=1, \\
        T^\gamma & \gamma<1.
    \end{cases}
\end{equation}
We further show that the entropy does not contain a residual term at $T=0$ (in contrast to certain SYK based models \cite{chowdhury_sachdev-ye-kitaev_2022}) and follows the same $T$-scaling as $C_v$. 


%It was already found \cite{riess_superconductivity_1980} that in the perturbative regime where uniformly distributed TLSs can lead to linear in $T$ resistivity, they also lead to parametric enhancement of $T_c$ relative to the (phonon-mediated) BCS form, due to the finite spectral weight of TLSs at small frequencies. Relying on these perturbative results, it may be that as the distribution is renormalized into the MFL and NFL regime $(\gamma\leq 1)$ the contribution of the TLSs to pairing will also change parametrically (due to the diverging spectral weight at low frequencies), constituting an enhanced mechanism for superconductivity. However, it is not obvious that this behavior will persist to strong coupling, and would furthermore not be effected by the broadening of the TLSs at intermediate couplings. The answer to this question requires an individual in depth study.






%such that changing the onsite disorder affects $\rho_0$ and does not alter the inelastic MFL (or NFL) behavior. 

%This is in line with experimental observations that show that the slope of the $T-$linear resistivity is unaffected by changing the amount of impurities [xx]. 

%Even in the absence of impurities, our theory generically generates an elastic scattering term due to frozen TLSs (which is small  

%, and in contrast to theories where the origin of $T-$linear resistivity is physically correlated with quenched disorder or originates from a clean `incoherent' conductivity.



%namely, changing the amount of impurities and cleanliness of the material will effect the elastic value $\rho_0$, it will not have significant effect on the inelastic NFL resistivity.


%Whether quenched disorder is necessary for strange metallicity is a question of ongoing debate. On the one hand, it is well-known that, in some strange metals [xx], adding impurities does not change the slope of the $T-$linear part of the resistivity. This makes scenarios in which the source of the $T-$linear resistivity is inherited from impurities -- and hence correlated with the disorder -- somewhat unnatural (i.e. if it is generated from disorder in the RG-sense). On the other hand, obtaining a $T-$linear resistivity in clean and controlled theories is incredibly challenging. Our framework provides a middle ground: although we find disorder necessary, the disorder in our case in annealed, and not quenched, and is generated intrinsically by the high degree of frustration in the system. In other words, the two types of disorder in our theory (i.e. $V_{ij,\vec{r}}$ and $\vec{g}_{ijl,\vec{r}}$) are naturally decoupled. Thus, while changing the amount of impurities and cleanliness of the material will effect the elastic value $\rho_0$, it will not have significant effect on the inelastic NFL resistivity. WF comment.


%with recent studies claiming that it lies in the heart of In particular, a seriesIn the context of QCP-related strange metallicity, it has been claimed that quenched disorder is necessary \cite{patel_universal_2023}, while others advocate for an intrinsic, independent of the presence of impurities [Else gifts and loop currents papers, other Senthil works?]. 



%has been in the heart of the debate Previous works describing strange metal phases in the context of QCPs have claimed that disorder is an essential ingredient for $T$ linear resistivity. On the other hand, others claim that MFL behavior should be an intrinsic property of the material, and does not scale with impurities and disorder. 


\begin{comment}
    
Talking points:
\begin{itemize}
    \item Quantum oscillations - new Subir paper \url{https://arxiv.org/abs/2308.01956}
    \item Superconductivity - Old TLS paper \url{https://www.sciencedirect.com/science/article/abs/pii/0375960180903631}
    \item a comment on inelastic vs. elastic $T-$linear resistivity? mention Das Sarma TBG phonons or Fernandez phasons and maybe mention WF criterion that can distinguish the two...
\end{itemize}

Supporting experimental evidence:...
\begin{itemize}
    \item Dessau \url{https://arxiv.org/abs/1509.01611}
    \item Ramshaw Isotropic paper
    \item Abbamonte EELS papers
    \item new LSCO paper \url{https://arxiv.org/pdf/2307.13740.pdf}
\end{itemize}
\end{comment}

